Compute--Forward Multiple Access (CFMA): Practical Code Design

We present a practical strategy that aims to attain rate points on the dominant face of the multiple access channel capacity using a standard low complexity decoder. This technique is built upon recent theoretical developments of Zhu and Gastpar on compute-forward multiple access (CFMA) which achieves the capacity of the multiple access channel using a sequential decoder. We illustrate this strategy with off-the-shelf LDPC codes. In the first stage of decoding, the receiver first recovers a linear combination of the transmitted codewords using the sum-product algorithm (SPA). In the second stage, by using the recovered sum-of-codewords as side information, the receiver recovers one of the two codewords using a modified SPA, ultimately recovering both codewords. The main benefit of recovering the sum-of-codewords instead of the codeword itself is that it allows to attain points on the dominant face of the multiple access channel capacity without the need of rate-splitting or time sharing while maintaining a low complexity in the order of a standard point-to-point decoder. This property is also shown to be crucial for some applications, e.g., interference channels. For all the simulations with single-layer binary codes, our proposed practical strategy is shown to be within \SI{1.7}{\decibel} of the theoretical limits, without explicit optimization on the off-the-self LDPC codes.

==> obsolete/16QAM-CFMA.tex <==
\begin{tikzpicture}
\begin{axis}[
xmin=3,
xmax=4,
xlabel={$r_1$},
ymin=3,
ymax=4,
ylabel={$r_2$},
xmajorgrids, 
ymajorgrids,
yminorgrids,
xminorgrids,
legend style={at={(0.109,0.109)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]

\addplot [color=red, line width=1.5pt]
  table[row sep=crcr]{%
3.99999963676631	0\\
3.99999963676631	3.41914661819364\\
3.86408938451388	3.55505687044607\\
3.55505687044607	3.55505687044607\\
3.55505687044607	3.86408938451388\\
3.41914661898605	3.9999996359739\\
0	3.9999996359739\\
};
\addlegendentry{binary input linear code}

\addplot [color=blue, line width=1.0pt]
  table[row sep=crcr]{%
3.99999963676631	0\\
3.99999963676631	3.41914661819364\\
3.41914661898605	3.9999996359739\\
0	3.9999996359739\\
};
\addlegendentry{binary input mac}

\addplot [color=green, line width=1.0pt]
  table[row sep=crcr]{%
3.55505687044607	0\\
3.55505687044607	3.55505687044607\\
0	3.55505687044607\\
};
\addlegendentry{binary input cf}
\end{axis}
\fill[latex-latex, thin, draw=black, fill=black] (5.93,3.16) circle(2pt);
\draw[black] (4.5,2.7) node[text width=3cm, align=right]{$(3.864,3.555)$};
\end{tikzpicture}

==> obsolete/4PAM-CFMA.tex <==
\begin{figure}[h]
\begin{tikzpicture}
\begin{axis}[
xmin=0,
xmax=2.1,
xlabel={$R_1$},
ymin=0,
ymax=2.1,
ylabel={$R_2$},
xmajorgrids, 
ymajorgrids,
yminorgrids,
xminorgrids,
legend style={at={(0.101,0.124)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]

\addplot [color=red, line width=1.5pt]
  table[row sep=crcr]{%
2.00000000000009	0\\
2.00000000000009	0.655639062229606\\
1.65563906222937	1.00000000000032\\
1.00000000000032	1.00000000000032\\
1.00000000000032	1.65563906222937\\
0.655639062229606	2.00000000000009\\
0	2.00000000000009\\
};
\addlegendentry{Binary input linear code}

\addplot [color=blue, line width=1.0pt]
  table[row sep=crcr]{%
2.00000000000009	0\\
2.00000000000009	0.655639062229606\\
0.655639062229606	2.00000000000009\\
0	2.00000000000009\\
};
\addlegendentry{Binary input MAC}

\addplot [color=green, line width=1.0pt]
  table[row sep=crcr]{%
1.65563906222937	0\\
1.65563906222937	1.65563906222937\\
0	1.65563906222937\\
};

\addlegendentry{Binary input CF}
\end{axis}
\end{tikzpicture}
\caption{Rate regions for bitwise sum}
\end{figure}

==> obsolete/SPA.tex <==
\section{The sum-product algorithm (SPA)}
\label{app:SPA}

The sum-product algorithm is an efficient algorithm for decoding binary LDPC codes.

\comment{Erixhen: please complete the SPA, use time index $i$ in the algorithm. -J}
\begin{algorithm}[h]
\caption{The sum-product algorithm (SPA)}
\begin{algorithmic}[1]
\Procedure{SPA}{$\ve H, \LLR$}
\State{\# (Define notations here)}
$\mu_{f\rightarrow s}(0)=\LLR_1$ \Comment{Initialization}
\For{$i=1$ to $N$} 
	%\State{$\mu_{f \rightarrow s} \gets \LLR_1$}
	\For{$\forall s$}
		\State $\mu_{s \rightarrow f}\gets \prod_{h \in n(s) \backslash \left\{f\right\}} \mu_{h \rightarrow s}$
	\EndFor
	\For{$\forall f$}
		\State $\mu_{f \rightarrow s} \gets \sum_{\sim \left\{s\right\}} \left( f(S) \prod_{y \in n(f) \backslash \left\{s\right\}} \mu_{y \rightarrow f} \right)$
	\EndFor
	\State \textbf{return} $\prod_{h \in n(s)} \mu_{h \rightarrow s}$\Comment{Soft decision for sum}
\EndFor
% \For{$i=1$ to $12$} \Comment{SPA{$(x,f)$}}
%    \State{$\mu_{f \rightarrow x} \gets \LLR_2$}
%    \For{$\forall x$}
%       \State $\mu_{x \rightarrow f}\gets \prod_{h \in n(x) \backslash \left\{f\right\}} \mu_{h \rightarrow x}$
%    \EndFor
%    \For{$\forall f$}
%       \State $\mu_{f \rightarrow x} \gets \sum_{\sim \left\{x\right\}} \left( f(X) \prod_{y \in n(f) \backslash \left\{x\right\}} \mu_{y \rightarrow f} \right)$
%    \EndFor
%    \State \textbf{return} $\prod_{h \in n(x)} \mu_{h \rightarrow x}$\Comment{Soft decision for a user}
% \EndFor
 \EndProcedure			
\end{algorithmic}
\label{alg:cfma}
\end{algorithm}
